Inference with Many Weak Instruments and Heterogeneity

This paper considers inference in a linear instrumental variable regression model with many potentially weak instruments, in the presence of heterogeneous treatment effects. I first show that existing test procedures, including those that are robust to either weak instruments or heterogeneous treatment effects, can be arbitrarily oversized. I propose a novel and valid test based on a score statistic and a ``leave-three-out" variance estimator. In the presence of heterogeneity and within the class of tests that are functions of the leave-one-out analog of a maximal invariant, this test is asymptotically the uniformly most powerful unbiased test. In two applications to judge and quarter-of-birth instruments, the proposed inference procedure also yields a bounded confidence set while some existing methods yield unbounded or empty confidence sets.

==> fig/ResMat.tex <==

\begin{tabular}{lrrrrrrr}
\toprule
  & rejLMorc & rejMO & rejL3O & rejAR & rejTSLS & rejJIVE & rejJIVEC\\
\midrule
base & 0.052 & 0.127 & 0.051 & 1.000 & 0.400 & 0.049 & 0.628\\
xi=0 & 0.053 & 0.046 & 0.053 & 0.041 & 0.923 & 0.111 & 0.021\\
p1=0 & 0.051 & 0.212 & 0.046 & 1.000 & 0.400 & 0.040 & 0.662\\
p1=1/2 & 0.051 & 0.055 & 0.057 & 0.046 & 0.350 & 0.106 & 0.016\\
S=9 & 0.052 & 0.078 & 0.045 & 1.000 & 0.233 & 0.052 & 0.394\\
S=1 & 0.052 & 0.169 & 0.054 & 1.000 & 0.451 & 0.041 & 0.306\\
\bottomrule
\end{tabular}


==> fig/Res_binX.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & rejLMorc & rejL3O & rejMO & rejMS & rejTSLS & rejEK & rejJIVEC & rejARC\\
\midrule
base & 0.052 & 0.051 & 0.127 & 1.000 & 0.400 & 0.049 & 0.628 & 0.124\\
xi=0 & 0.053 & 0.053 & 0.046 & 0.041 & 0.923 & 0.111 & 0.021 & 0.047\\
$S=\sqrt{K}(c-1).5$ & 0.054 & 0.042 & 0.042 & 1.000 & 0.107 & 0.042 & 0.070 & 0.041\\
$S=.1,\xi=0,\sigma_{\varepsilon \varepsilon}=0$ & 0.054 & 0.058 & 0.069 & 0.054 & 1.000 & 0.722 & 0.805 & 0.153\\
$S=0,\xi=0,\sigma_{\varepsilon \varepsilon}=0$ & 0.049 & 0.044 & 0.064 & 0.049 & 1.000 & 1.000 & 1.000 & 0.149\\
\bottomrule
\end{tabular}


==> fig/Res_contX.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & rejLMorc & rejL3O & rejMO & rejMS & rejTSLS & rejEK & rejJIVEC & rejARC\\
\midrule
base & 0.051 & 0.054 & 0.154 & 1.000 & 1.000 & 0.008 & 0.605 & 0.150\\
ConTE & 0.043 & 0.055 & 0.064 & 0.044 & 1.000 & 0.157 & 0.188 & 0.146\\
$S=3\sqrt{K}$ & 0.053 & 0.061 & 0.095 & 1.000 & 0.954 & 0.023 & 0.134 & 0.099\\
S=.1,$\sigma_{\varepsilon v}=1$,ConTE & 0.052 & 0.054 & 0.076 & 0.051 & 1.000 & 0.768 & 0.954 & 0.167\\
S=0,$\sigma_{\varepsilon v}=1$,ConTE & 0.053 & 0.056 & 0.072 & 0.053 & 1.000 & 1.000 & 1.000 & 0.144\\
\bottomrule
\end{tabular}


==> fig/Res_contX_hetsked.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & rejLMorc & rejL3O & rejMO & rejMS & rejTSLS & rejEK & rejJIVEC & rejARC\\
\midrule
base & 0.049 & 0.054 & 0.059 & 0.062 & 1.000 & 0.029 & 0.039 & 0.068\\
fixsigxiv & 0.060 & 0.054 & 0.088 & 0.995 & 0.999 & 0.010 & 0.058 & 0.092\\
ConTE & 0.055 & 0.056 & 0.062 & 0.053 & 1.000 & 0.100 & 0.074 & 0.075\\
S=3*sqrt(K) & 0.048 & 0.046 & 0.053 & 0.692 & 0.753 & 0.023 & 0.055 & 0.053\\
S=.1,sigev=1,ConTE & 0.046 & 0.052 & 0.070 & 0.048 & 1.000 & 0.741 & 0.952 & 0.153\\
\addlinespace
S=0,sigev=1,ConTE & 0.050 & 0.045 & 0.061 & 0.050 & 1.000 & 1.000 & 1.000 & 0.147\\
\bottomrule
\end{tabular}


==> fig/S4sim_binX_res.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & rejTSLS & rejEK & rejMS & rejMO & rejJIVEC & rejARC & rejL3O & rejLMorc\\
\midrule
weakIV,weakHet & 0.229 & 0.079 & 0.394 & 0.064 & 0.022 & 0.067 & 0.056 & 0.051\\
weakIV,weakHet,sigev=.5 & 0.992 & 0.121 & 0.164 & 0.065 & 0.071 & 0.088 & 0.068 & 0.047\\
weakIV,strongHet & 0.170 & 0.048 & 0.999 & 0.093 & 0.034 & 0.090 & 0.050 & 0.045\\
strongIV,weakHet & 0.053 & 0.049 & 0.059 & 0.037 & 0.036 & 0.039 & 0.043 & 0.041\\
strongIV,weakHet,sigev=.5 & 0.187 & 0.064 & 0.057 & 0.045 & 0.044 & 0.051 & 0.053 & 0.048\\
\addlinespace
strongIV,strongHet & 0.046 & 0.043 & 0.173 & 0.040 & 0.039 & 0.040 & 0.045 & 0.044\\
ConTE & 0.999 & 0.140 & 0.046 & 0.044 & 0.080 & 0.065 & 0.059 & 0.044\\
S=.1,sigev=1,ConTE & 1.000 & 0.456 & 0.051 & 0.076 & 0.503 & 0.139 & 0.082 & 0.058\\
S=0,sigev=1,ConTE & 1.000 & 0.527 & 0.055 & 0.067 & 0.590 & 0.142 & 0.078 & 0.052\\
\bottomrule
\end{tabular}


==> fig/S4sim_binX_stat.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & LM\_num & MOvar & AR\_num & L3OLMvar & TSLSt & JIVEt & JIVEtC & ARC\_num\\
\midrule
weakIV,weakHet & -0.0153576 & 0.3296046 & 0.8770807 & 0.3680810 & -1.1614219 & -0.0284549 & -0.1038597 & -0.0172054\\
weakIV,weakHet,sigev=.5 & 0.0037194 & 0.6371771 & 0.8474621 & 0.6986974 & -4.7146681 & -0.0494728 & -0.3330237 & 0.0405225\\
weakIV,strongHet & 0.0018743 & 0.9683465 & 8.8721750 & 1.3538757 & -0.6443795 & -0.0069659 & -0.0434949 & 0.0092334\\
strongIV,weakHet & -0.0176217 & 0.6695442 & 0.1396228 & 0.6605973 & -0.3234061 & -0.0188936 & -0.0217218 & -0.0178878\\
strongIV,weakHet,sigev=.5 & 0.0910652 & 1.1617640 & 0.1452159 & 1.1593671 & -1.0793973 & 0.0935834 & 0.0755671 & 0.0924902\\
\addlinespace
strongIV,strongHet & 0.0419611 & 2.0156159 & 1.4275635 & 1.9084130 & -0.1354545 & 0.0299894 & 0.0274347 & 0.0300256\\
ConTE & -0.0008133 & 0.5658187 & -0.0069990 & 0.6141160 & -5.1598940 & -0.0561443 & -0.3643065 & 0.0305191\\
S=.1,sigev=1,ConTE & 0.0293651 & 1.5106430 & -0.0277028 & 1.7668785 & -16.0493050 & -2.2101848 & -2.1863340 & 0.0910302\\
S=0,sigev=1,ConTE & -0.0847069 & 1.5639723 & 0.0753641 & 1.8242340 & -20.1371951 & -2.8121303 & -2.6515009 & -0.0272775\\
\bottomrule
\end{tabular}


==> fig/S4sim_contX_res.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & rejTSLS & rejEK & rejMS & rejMO & rejJIVEC & rejARC & rejL3O & rejLMorc\\
\midrule
weakIV,weakHet & 0.069 & 0.021 & 0.397 & 0.055 & 0.017 & 0.052 & 0.046 & 0.046\\
weakIV,weakHet,$\sigma_{\varepsilon v}=.5$ & 1.000 & 0.043 & 0.388 & 0.077 & 0.074 & 0.087 & 0.057 & 0.056\\
weakIV,strongHet & 0.157 & 0.003 & 1.000 & 0.168 & 0.068 & 0.139 & 0.059 & 0.051\\
\addlinespace
strongIV,weakHet & 0.069 & 0.048 & 0.351 & 0.069 & 0.068 & 0.069 & 0.061 & 0.050\\
strongIV,weakHet,$\sigma_{\varepsilon v}=.5$ & 0.991 & 0.039 & 0.374 & 0.053 & 0.056 & 0.054 & 0.044 & 0.052\\
strongIV,strongHet & 0.092 & 0.014 & 1.000 & 0.096 & 0.092 & 0.090 & 0.048 & 0.044\\
\addlinespace
ConTE & 1.000 & 0.103 & 0.053 & 0.056 & 0.081 & 0.077 & 0.047 & 0.048\\
S=.1,$\sigma_{\varepsilon v}=1$,ConTE & 1.000 & 0.769 & 0.053 & 0.078 & 0.963 & 0.171 & 0.068 & 0.054\\
S=0,$\sigma_{\varepsilon v}=1$,ConTE & 1.000 & 1.000 & 0.054 & 0.077 & 1.000 & 0.158 & 0.058 & 0.054\\
\bottomrule
\end{tabular}


==> fig/sim_binX_res.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & TSLS & EK & MS & MO & JIVEC & ARC & L3O & LMorc\\
\midrule
weakIV,weakHet & 0.217 & 0.075 & 0.414 & 0.065 & 0.029 & 0.068 & 0.066 & 0.058\\
weakIV,weakHet,$\sigma_{\varepsilon v}=.5$ & 0.994 & 0.112 & 0.186 & 0.069 & 0.068 & 0.083 & 0.079 & 0.045\\
weakIV,strongHet & 0.168 & 0.060 & 0.999 & 0.099 & 0.031 & 0.095 & 0.061 & 0.047\\
strongIV,weakHet & 0.059 & 0.049 & 0.062 & 0.037 & 0.039 & 0.040 & 0.043 & 0.044\\
strongIV,weakHet,$\sigma_{\varepsilon v}=.5$ & 0.227 & 0.069 & 0.065 & 0.050 & 0.055 & 0.054 & 0.057 & 0.047\\
\addlinespace
strongIV,strongHet & 0.056 & 0.053 & 0.183 & 0.043 & 0.042 & 0.043 & 0.050 & 0.048\\
ConTE & 0.996 & 0.154 & 0.053 & 0.052 & 0.082 & 0.079 & 0.070 & 0.042\\
S=1,$\sigma_{\varepsilon v}=1$,ConTE & 1.000 & 0.278 & 0.054 & 0.073 & 0.288 & 0.131 & 0.082 & 0.053\\
S=0,$\sigma_{\varepsilon v}=1$,ConTE & 1.000 & 0.549 & 0.047 & 0.070 & 0.605 & 0.156 & 0.075 & 0.056\\
\bottomrule
\end{tabular}


==> fig/sim_binX_stat.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & LM\_num & MOvar & AR\_num & L3OLMvar & TSLSt & JIVEt & JIVEtC & ARC\_num\\
\midrule
weakIV,weakHet & 0.0044707 & 0.3317703 & 0.8802532 & 0.3710664 & -1.0895185 & 0.0099222 & -0.0720678 & 0.0166215\\
weakIV,weakHet,sigev=.5 & 0.0259757 & 0.6412975 & 0.8677233 & 0.7111162 & -4.6862251 & -0.0420391 & -0.3351926 & 0.0673200\\
weakIV,strongHet & 0.0115348 & 0.9627310 & 8.9213729 & 1.3475380 & -0.6280690 & -0.0163818 & -0.0459354 & 0.0191744\\
strongIV,weakHet & 0.0033785 & 0.6700751 & 0.1347642 & 0.6556482 & -0.3004021 & 0.0069308 & 0.0023528 & 0.0070088\\
strongIV,weakHet,sigev=.5 & -0.0066073 & 1.1638285 & 0.1516791 & 1.1578964 & -1.1644931 & -0.0011905 & -0.0142322 & 0.0036324\\
\addlinespace
strongIV,strongHet & -0.0933141 & 2.0155683 & 1.4602945 & 1.8991087 & -0.2424798 & -0.0701374 & -0.0691592 & -0.0660352\\
ConTE & 0.0370925 & 0.5663765 & -0.0027787 & 0.5961456 & -5.0882951 & -0.0251198 & -0.3448930 & 0.0865013\\
S=1,sigev=1,ConTE & -0.0326499 & 1.4742191 & 0.0441383 & 1.6622060 & -10.6330410 & -1.1067164 & -1.3443461 & 0.0229008\\
S=0,sigev=1,ConTE & -0.0997140 & 1.5606569 & 0.1256505 & 1.8249013 & -20.1935628 & -2.9160363 & -2.6870467 & -0.0379413\\
\bottomrule
\end{tabular}


==> fig/sim_binXcov_res.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & TSLS & EK & MS & MO & JIVEC & ARC & L3O & LMorc\\
\midrule
weakIV,weakHet & 0.158 & 0.023 & 0.100 & 0.060 & 0.006 & 0.061 & 0.060 & 0.058\\
weakIV,weakHet,$\sigma_{\varepsilon v}=.5$ & 0.940 & 0.084 & 0.072 & 0.043 & 0.060 & 0.066 & 0.055 & 0.049\\
weakIV,strongHet & 0.162 & 0.021 & 0.485 & 0.087 & 0.009 & 0.089 & 0.061 & 0.050\\
strongIV,weakHet & 0.075 & 0.133 & 0.046 & 0.045 & 0.045 & 0.049 & 0.053 & 0.049\\
strongIV,weakHet,$\sigma_{\varepsilon v}=.5$ & 0.317 & 0.110 & 0.048 & 0.048 & 0.042 & 0.053 & 0.058 & 0.045\\
\addlinespace
strongIV,strongHet & 0.036 & 0.107 & 0.042 & 0.032 & 0.029 & 0.032 & 0.031 & 0.046\\
ConTE & 0.146 & 0.014 & 0.048 & 0.047 & 0.007 & 0.047 & 0.059 & 0.042\\
S=1,$\sigma_{\varepsilon v}=1$,ConTE & 1.000 & 0.208 & 0.054 & 0.048 & 0.264 & 0.107 & 0.078 & 0.041\\
S=0,$\sigma_{\varepsilon v}=1$,ConTE & 1.000 & 0.323 & 0.040 & 0.042 & 0.409 & 0.133 & 0.089 & 0.041\\
\bottomrule
\end{tabular}


==> fig/sim_binXcov_stat.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & LM\_num & MOvar & AR\_num & L3OLMvar & TSLSt & JIVEt & JIVEtC & ARC\_num\\
\midrule
weakIV,weakHet & -0.0189447 & 0.5212398 & 0.3599024 & 0.5435410 & -0.8917311 & -0.1325959 & -0.1552308 & -0.0132429\\
weakIV,weakHet,sigev=.5 & -0.0313204 & 1.0856258 & 0.4093470 & 1.1242616 & -3.7426732 & -0.4547008 & -0.5592316 & 0.0231833\\
weakIV,strongHet & -0.0094039 & 1.0184831 & 2.6384080 & 1.2474633 & -0.6322772 & -0.1216484 & -0.1179561 & 0.0047519\\
strongIV,weakHet & -0.0437787 & 0.9922331 & -0.0136407 & 0.9680272 & -0.4393959 & -0.0776931 & -0.0465104 & -0.0390233\\
strongIV,weakHet,sigev=.5 & 0.0710033 & 1.7895971 & -0.0284076 & 1.7907292 & -1.4765314 & 0.0334895 & 0.0080393 & 0.0849993\\
\addlinespace
strongIV,strongHet & 0.0526339 & 1.9620930 & -0.0464657 & 1.9349372 & -0.2345214 & 0.0385569 & 0.0330375 & 0.0378990\\
ConTE & 0.0234092 & 0.4369434 & 0.0015658 & 0.4277377 & -0.9039085 & -0.1210463 & -0.1205726 & 0.0548486\\
S=1,sigev=1,ConTE & 0.0109564 & 2.7434750 & 0.0407114 & 2.7459429 & -7.3355678 & -1.0492845 & -1.3156047 & 0.0939884\\
S=0,sigev=1,ConTE & 0.0269224 & 2.9087775 & -0.0146905 & 2.8756688 & -9.7688691 & NaN & -1.8462533 & 0.1209357\\
\bottomrule
\end{tabular}


==> fig/sim_contX_res.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & TSLS & EK & MS & MO & JIVEC & ARC & L3O & LMorc\\
\midrule
weakIV,weakHet & 0.076 & 0.021 & 0.406 & 0.073 & 0.019 & 0.069 & 0.057 & 0.053\\
weakIV,weakHet,$\sigma_{\varepsilon v}=.5$ & 1.000 & 0.046 & 0.410 & 0.068 & 0.066 & 0.080 & 0.053 & 0.054\\
weakIV,strongHet & 0.153 & 0.002 & 1.000 & 0.158 & 0.063 & 0.130 & 0.059 & 0.053\\
strongIV,weakHet & 0.063 & 0.040 & 0.349 & 0.056 & 0.055 & 0.055 & 0.052 & 0.051\\
strongIV,weakHet,$\sigma_{\varepsilon v}=.5$ & 0.981 & 0.048 & 0.370 & 0.063 & 0.065 & 0.066 & 0.057 & 0.048\\
\addlinespace
strongIV,strongHet & 0.078 & 0.014 & 1.000 & 0.094 & 0.092 & 0.093 & 0.051 & 0.053\\
ConTE,$\sigma_{\varepsilon v}=.5$ & 1.000 & 0.099 & 0.051 & 0.044 & 0.064 & 0.061 & 0.040 & 0.043\\
S=1,$\sigma_{\varepsilon v}=1$,ConTE & 1.000 & 0.342 & 0.053 & 0.074 & 0.593 & 0.161 & 0.059 & 0.054\\
S=0,$\sigma_{\varepsilon v}=1$,ConTE & 1.000 & 1.000 & 0.052 & 0.070 & 1.000 & 0.164 & 0.054 & 0.052\\
\bottomrule
\end{tabular}


==> fig/sim_contX_res_K40.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & TSLS & EK & MS & MO & JIVEC & ARC & L3O & LMorc\\
\midrule
weakIV,weakHet & 0.077 & 0.027 & 0.243 & 0.069 & 0.026 & 0.070 & 0.061 & 0.048\\
weakIV,weakHet,$\sigma_{\varepsilon v}=.5$ & 0.483 & 0.039 & 0.212 & 0.073 & 0.063 & 0.082 & 0.064 & 0.051\\
weakIV,strongHet & 0.164 & 0.023 & 0.861 & 0.147 & 0.074 & 0.133 & 0.065 & 0.058\\
strongIV,weakHet & 0.080 & 0.043 & 0.187 & 0.067 & 0.072 & 0.071 & 0.057 & 0.052\\
strongIV,weakHet,$\sigma_{\varepsilon v}=.5$ & 0.193 & 0.035 & 0.181 & 0.056 & 0.065 & 0.069 & 0.051 & 0.054\\
\addlinespace
strongIV,strongHet & 0.081 & 0.020 & 0.801 & 0.078 & 0.095 & 0.084 & 0.044 & 0.061\\
ConTE,$\sigma_{\varepsilon v}=.5$ & 0.794 & 0.085 & 0.049 & 0.053 & 0.061 & 0.083 & 0.084 & 0.046\\
S=1,$\sigma_{\varepsilon v}=1$,ConTE & 1.000 & 0.311 & 0.047 & 0.060 & 0.588 & 0.171 & 0.084 & 0.047\\
S=0,$\sigma_{\varepsilon v}=1$,ConTE & 1.000 & 1.000 & 0.044 & 0.056 & 1.000 & 0.179 & 0.090 & 0.044\\
\bottomrule
\end{tabular}


==> fig/sim_contX_stat.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & LM\_num & MOvar & AR\_num & L3OLMvar & TSLSt & JIVEt & JIVEtC & ARC\_num\\
\midrule
weakIV,weakHet & 0.0387416 & 1.121693 & 3.0455413 & 1.228965 & 0.0193010 & 0.0213537 & 0.0275283 & 0.0378446\\
weakIV,weakHet,sigev=.5 & 0.0000088 & 1.258320 & 3.0101060 & 1.426729 & 9.6441042 & 0.1477044 & 0.3146433 & -0.0149740\\
weakIV,strongHet & -0.1158193 & 2.596271 & 67.1406027 & 4.994478 & -0.0857277 & -0.0291192 & -0.0404827 & -0.0669115\\
strongIV,weakHet & -0.0275606 & 4.419161 & 3.0339360 & 4.605838 & -0.0247820 & -0.0140804 & -0.0138016 & -0.0136232\\
strongIV,weakHet,sigev=.5 & 0.0323290 & 4.556532 & 3.0563119 & 4.818342 & 4.2337038 & 0.0101115 & 0.0185669 & 0.0026501\\
\addlinespace
strongIV,strongHet & -0.1047663 & 12.616751 & 66.9710398 & 16.859026 & -0.0285816 & -0.0209304 & -0.0317477 & -0.0315844\\
ConTE,sigev=.5 & 0.0149714 & 1.046982 & -0.0065165 & 1.114952 & 11.8911535 & 0.2673935 & 0.3599303 & 0.0013074\\
S=1,sigev=1,ConTE & 0.0703865 & 1.382742 & 0.0628797 & 1.655411 & 200.9930745 & 1.9000028 & 3.8300770 & 0.0438603\\
S=0,sigev=1,ConTE & 0.0566094 & 1.346496 & 0.0566094 & 1.600236 & Inf & Inf & Inf & 0.0332485\\
\bottomrule
\end{tabular}


==> fig/sim_contX_stat_K40.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & LM\_num & MOvar & AR\_num & L3OLMvar & TSLSt & JIVEt & JIVEtC & ARC\_num\\
\midrule
weakIV,weakHet & -0.0240835 & 1.873617 & 3.0862539 & 2.333039 & -0.0450071 & 0.0000607 & 0.0144568 & -0.0208630\\
weakIV,weakHet,sigev=.5 & 0.0399822 & 2.028471 & 2.9775270 & 2.509936 & 2.0212569 & 0.0999432 & 0.3011766 & -0.0212710\\
weakIV,strongHet & 0.1022244 & 3.670155 & 18.8676232 & 6.236638 & 0.0373974 & 0.0399784 & 0.0525155 & 0.0580148\\
strongIV,weakHet & -0.0384870 & 5.920671 & 2.9939235 & 6.626007 & -0.0119926 & -0.0205207 & -0.0206696 & -0.0187257\\
strongIV,weakHet,sigev=.5 & -0.0060705 & 5.992405 & 2.9736530 & 6.819390 & 1.0289228 & -0.0118437 & 0.0056956 & -0.0438383\\
\addlinespace
strongIV,strongHet & 0.1271772 & 12.753655 & 19.1565966 & 17.036227 & 0.0304941 & 0.0254342 & 0.0392307 & 0.0374787\\
ConTE,sigev=.5 & 0.0069065 & 1.334672 & 0.0269593 & 1.396939 & 2.8960188 & 0.2584749 & 0.3746966 & -0.0483634\\
S=1,sigev=1,ConTE & -0.0109901 & 1.493582 & -0.0125851 & 1.754050 & 27.6358746 & 1.6939452 & 3.6310413 & -0.1155844\\
S=0,sigev=1,ConTE & 0.0035864 & 1.388718 & 0.0035864 & 1.672689 & Inf & Inf & Inf & -0.1079786\\
\bottomrule
\end{tabular}


==> fig/sim_example_fixedK_res.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & TSLS & EK & MS & MO & JIVEC & ARC & L3O & LMorc\\
\midrule
$C_H=.5c$,$C_S=.5c$ & 0.325 & 0.050 & 1.000 & 0.318 & 0.324 & 0.323 & 0.056 & 0.051\\
$C_H=.5c$,$C_S=2$ & 0.575 & 0.012 & 1.000 & 0.820 & 0.277 & 0.833 & 0.040 & 0.047\\
$C_H=.5c$,$C_S=0$ & 0.501 & 0.005 & 1.000 & 0.856 & 0.335 & 0.881 & 0.061 & 0.050\\
\addlinespace
$C_H=2$,$C_S=.5c$ & 0.082 & 0.057 & 0.604 & 0.081 & 0.073 & 0.082 & 0.065 & 0.060\\
$C_H=2$,$C_S=2$ & 0.485 & 0.013 & 0.625 & 0.348 & 0.326 & 0.466 & 0.109 & 0.046\\
$C_H=2$,$C_S=0$ & 0.461 & 0.011 & 0.624 & 0.341 & 0.349 & 0.497 & 0.107 & 0.047\\
\addlinespace
$C_H=0$,$C_S=.5c$ & 0.064 & 0.045 & 0.043 & 0.044 & 0.046 & 0.051 & 0.055 & 0.043\\
$C_H=0$,$C_S=2$ & 0.437 & 0.102 & 0.048 & 0.040 & 0.296 & 0.134 & 0.066 & 0.042\\
$C_H=0$,$C_S=0$ & 0.590 & 0.181 & 0.049 & 0.029 & 0.431 & 0.163 & 0.059 & 0.045\\
\bottomrule
\end{tabular}


==> fig/sim_example_power_res.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & TSLS & EK & MS & MO & JIVEC & ARC & L3O & LMorc\\
\midrule
$C_H=2\sqrt{K}$,$C_S=2\sqrt{K}$ & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
$C_H=2\sqrt{K}$,$C_S=2$ & 0.449 & 0.100 & 1.000 & 0.463 & 0.044 & 0.452 & 0.179 & 0.153\\
$C_H=2\sqrt{K}$,$C_S=0$ & 0.825 & 0.028 & 1.000 & 0.305 & 0.063 & 0.298 & 0.050 & 0.043\\
\addlinespace
$C_H=3$,$C_S=3\sqrt{K}$ & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
$C_H=3$,$C_S=3$ & 0.322 & 0.491 & 1.000 & 0.881 & 0.150 & 0.889 & 0.737 & 0.752\\
$C_H=3$,$C_S=0$ & 1.000 & 0.080 & 1.000 & 0.138 & 0.196 & 0.177 & 0.052 & 0.057\\
\addlinespace
$C_H=0$,$C_S=2\sqrt{K}$ & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
$C_H=0$,$C_S=2$ & 0.881 & 0.400 & 0.978 & 0.776 & 0.075 & 0.812 & 0.692 & 0.752\\
$C_H=0$,$C_S=0$ & 1.000 & 0.366 & 0.046 & 0.049 & 0.322 & 0.092 & 0.061 & 0.049\\
\bottomrule
\end{tabular}


==> fig/sim_example_res.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & TSLS & EK & MS & MO & JIVEC & ARC & L3O & LMorc\\
\midrule
$C_H=2\sqrt{K}$,$C_S=2\sqrt{K}$ & 0.900 & 0.066 & 1.000 & 0.103 & 0.100 & 0.101 & 0.055 & 0.053\\
$C_H=2\sqrt{K}$,$C_S=2$ & 1.000 & 0.033 & 1.000 & 0.285 & 0.076 & 0.271 & 0.045 & 0.045\\
$C_H=2\sqrt{K}$,$C_S=0$ & 0.998 & 0.024 & 1.000 & 0.308 & 0.055 & 0.297 & 0.051 & 0.048\\
\addlinespace
$C_H=3$,$C_S=3\sqrt{K}$ & 0.996 & 0.066 & 1.000 & 0.042 & 0.043 & 0.044 & 0.039 & 0.048\\
$C_H=3$,$C_S=3$ & 1.000 & 0.101 & 1.000 & 0.101 & 0.181 & 0.141 & 0.056 & 0.057\\
$C_H=3$,$C_S=0$ & 1.000 & 0.141 & 1.000 & 0.133 & 0.242 & 0.192 & 0.069 & 0.054\\
\addlinespace
$C_H=0$,$C_S = 2\sqrt{K}$ & 1.000 & 0.145 & 0.048 & 0.064 & 0.074 & 0.074 & 0.064 & 0.052\\
$C_H=0$,$C_S=2$ & 1.000 & 0.248 & 0.043 & 0.063 & 0.217 & 0.105 & 0.046 & 0.057\\
$C_H=0$,$C_S=0$ & 1.000 & 0.378 & 0.044 & 0.066 & 0.337 & 0.128 & 0.064 & 0.050\\
\bottomrule
\end{tabular}


==> fig/simf_example_fixedK_res.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & TSLS & EK &$T_{ee}$(MS) & $T_{eX}$(MO)  & $\tilde{X}$-t & $\tilde{X}$-AR & L3O & LMorc\\
\midrule
$C_H=.5c,C_S=.5c$ & 0.325 & 0.050 & 1.000 & 0.316 & 0.324 & 0.323 & 0.056 & 0.051\\
$C_H=.5c,C_S=2$ & 0.575 & 0.012 & 1.000 & 0.820 & 0.277 & 0.833 & 0.040 & 0.047\\
$C_H=.5c,C_S=0$ & 0.501 & 0.005 & 1.000 & 0.856 & 0.335 & 0.881 & 0.061 & 0.050\\
\addlinespace
$C_H=2,C_S=.5c$ & 0.082 & 0.057 & 0.604 & 0.081 & 0.073 & 0.082 & 0.065 & 0.060\\
$C_H=2,C_S=2$ & 0.485 & 0.013 & 0.625 & 0.347 & 0.326 & 0.466 & 0.109 & 0.046\\
$C_H=2,C_S=0$ & 0.461 & 0.011 & 0.624 & 0.341 & 0.349 & 0.497 & 0.107 & 0.047\\
\addlinespace
$C_H=0,C_S=.5c$ & 0.064 & 0.045 & 0.043 & 0.044 & 0.046 & 0.051 & 0.055 & 0.043\\
$C_H=0,C_S=2$  & 0.437 & 0.102 & 0.048 & 0.040 & 0.296 & 0.134 & 0.066 & 0.042\\
$C_H=0,C_S=0$  & 0.590 & 0.181 & 0.049 & 0.029 & 0.431 & 0.163 & 0.059 & 0.045\\
\bottomrule
\end{tabular}


==> fig/simf_example_power_res.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & TSLS & EK & $T_{ee}$(MS) & $T_{eX}$(MO)  & $\tilde{X}$-t & $\tilde{X}$-AR & L3O & LMorc\\
\midrule
$C_H=2\sqrt{K}, C_S = 2\sqrt{K}$ & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
$C_H=2\sqrt{K}, C_S = 2$& 0.449 & 0.100 & 1.000 & 0.417 & 0.044 & 0.452 & 0.179 & 0.153\\
$C_H=2\sqrt{K}, C_S = 0$ & 0.825 & 0.028 & 1.000 & 0.273 & 0.063 & 0.298 & 0.050 & 0.043\\
\addlinespace
$C_H=3, C_S = 3\sqrt{K}$ & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
$C_H=3, C_S = 3$ & 0.322 & 0.491 & 1.000 & 0.865 & 0.150 & 0.889 & 0.737 & 0.752\\
$C_H=3, C_S = 0$ & 1.000 & 0.080 & 1.000 & 0.109 & 0.196 & 0.177 & 0.052 & 0.057\\
\addlinespace
$C_H=0, C_S = 2\sqrt{K}$ & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000\\
$C_H=0, C_S = 2$ & 0.881 & 0.400 & 0.978 & 0.747 & 0.075 & 0.812 & 0.692 & 0.752\\
$C_H=0, C_S = 0$ & 1.000 & 0.366 & 0.046 & 0.033 & 0.322 & 0.092 & 0.061 & 0.049\\
\bottomrule
\end{tabular}


==> fig/simf_example_res.tex <==

\begin{tabular}{lrrrrrrrr}
\toprule
  & TSLS & EK & $T_{ee}$(MS) & $T_{eX}$(MO)  & $\tilde{X}$-t & $\tilde{X}$-AR & L3O & LMorc\\
\midrule
$C_H=2\sqrt{K}, C_S = 2\sqrt{K}$ & 0.900 & 0.066 & 1.000 & 0.078 & 0.100 & 0.101 & 0.055 & 0.053\\
$C_H=2\sqrt{K}, C_S = 2$ & 1.000 & 0.033 & 1.000 & 0.248 & 0.076 & 0.271 & 0.045 & 0.045\\
$C_H=2\sqrt{K}, C_S = 0$ & 0.998 & 0.024 & 1.000 & 0.264 & 0.055 & 0.297 & 0.051 & 0.048\\
\addlinespace
$C_H=3, C_S = 3\sqrt{K}$ & 0.996 & 0.066 & 1.000 & 0.036 & 0.043 & 0.044 & 0.039 & 0.048\\
$C_H=3, C_S = 3$ & 1.000 & 0.101 & 1.000 & 0.084 & 0.181 & 0.141 & 0.056 & 0.057\\
$C_H=3, C_S = 0$ & 1.000 & 0.141 & 1.000 & 0.107 & 0.242 & 0.192 & 0.069 & 0.054\\
\addlinespace
$C_H=0, C_S = 2\sqrt{K}$ & 1.000 & 0.145 & 0.048 & 0.058 & 0.074 & 0.074 & 0.064 & 0.052\\
$C_H=0, C_S = 2$ & 1.000 & 0.248 & 0.043 & 0.048 & 0.217 & 0.105 & 0.046 & 0.057\\
$C_H=0, C_S = 0$ & 1.000 & 0.378 & 0.044 & 0.058 & 0.337 & 0.128 & 0.064 & 0.050\\
\bottomrule
\end{tabular}

